Multiwavelength Modeling for the Shallow Decay Phase of Gamma-Ray Burst Afterglows

We simulate the emission in the shallow decay phase of gamma-ray burst afterglows using a time-dependent code. We test four models: the energy injection model, evolving the injection efficiency of non-thermal electrons, evolving the amplification of the magnetic field, and the wind model with a relatively low bulk Lorentz factor. All of the four models can reproduce the typical X-ray afterglow lightcurve. The spectral shape depends on not only the parameter values at the time corresponding to the observer time but also the past evolution of the parameters. The model differences appear in the evolution of the broadband spectrum, especially in the inverse Compton component. Future gamma-ray observations with imaging atmospheric Cherenkov telescopes such as CTA will reveal the mechanism of the shallow decay phase.

==> trash/ABSTRACT.tex <==
\begin{abstract}
We calculate the non-thermal emission from massive ($M_{500}>10^{14}M_\odot$) galaxy clusters and evaluate the contributions to the extragalactic radio and neutrino background observed by ARCADE 2 and IceCube, respectively.
The radio emission from galaxy clusters and its statistical properties are well explained with the scenario where the non-thermal particles are re-accelerated by merger-induced turbulence. 
We assume that the seed electrons for the re-acceleration is provided by $pp$ collision of cosmic-ray protons, and model the temporal evolutions of the radio and neutrino luminosities and their luminosity--mass relations.
We exploit the Monte Carlo merger tree to follow the history of cluster mergers and luminosity evolution, and construct the luminosity functions for radio and neutrino emission.
The model parameters, such as the threshold mass ratio for the onset of re-acceleration, are constrained by the statistical properties of observed giant radio halos.
We find that the contribution to the ARCADE 2 excess is marginal, contrary to the previous estimate. 
The clusters with $M_{500}>10^{15}M_\odot$ contributes most to the neutrino background, although it is only 5\% of the IceCube intensity in our fiducial model.
The contribution increases up to 20\% with an optimistic assumption on the neutrino luminosity--mass relation, whose radio contemporary can be tested by near-future radio halo survey.
\end{abstract}


%Extended radio structures found in a fraction of massive galaxy clusters proves the existence of relativistic particles in the intra-cluster space.
%We also construct the luminosity function for high-energy neutrinos, assuming that the seed electrons for the reacceleration is originated from the pp collision of high-energy protons. 

==> trash/CONCLUSION.tex <==
\section{Conclusions\label{sec:conclusion}}



%An increasing number of RHs have been found in recent radio observations of galaxy clusters. The correlation between RHs and dynamically disturbed clusters supports the scenario where the RH emission is powered by the reacceleration of CRs by the merger-induced turbulence, but the origin of the seed CREs for the reacceleration is still poorly constrained. In this study, we compare two possibilities for the origin; the secondary scenario, where the seed population is provided as secondary particles injected via the pp collision, and the primary scenario, where most of the seed CREs are originated from the background thermal electrons and the secondary injection from the pp collision is negligible. \par

%We have solved the FP equations to follow the evolution of the CR distribution in RHs. Our calculation method is basically the same as the one in \citet{paperI}, but we have newly included the radial dependence of the reacceleration efficiency in this paper. %We have assumed the hard-sphere type reacceleration, where parent CRPs are efficiently accelerated along with CREs. 
T%he radio and gamma-ray observations of the Coma cluster is used to constrain the model parameters. Assuming that the primary CRs are injected with the same radial profile as the thermal gas density, we have found that the radially increasing efficiency of the reacceleration reproduces both the radial profile and the spectrum of the Coma RH under the gamma-ray limit given by {\it Fermi}-LAT. \par 
%\ers{We have confirmed that radially increasing profile of the turbulence and the acceleration timescale of $t_{\rm acc}\approx300~{\rm Myr}$ reproduce both the profile and the spectrum of the RH under the gamma-ray limit given by Fermi-LAT.} \par

%Our model calibrated by the Coma RH is then used to study the lifetime of RHs in Section~\ref{sec:lifetime}. 
%We assumed that the reacceleration phase ends in $t_{\rm R}\approx500~{\rm Myr}$, and
We have followed the evolution in the cooling phase, where the reacceleration ceases. 
%\ers{by setting $D_{pp}=0$ in the FP equations.}
The main results in this part are summarized as follows:
\begin{itemize}
    \item There are two factors that powers the radio emission: the reacceleration of the seed CREs and the enhanced secondary injection from reaccelerated CRPs. 
    \item In the secondary scenario, a substantial part of the emission is produced by the injection from reaccelerated CRPs. This emission lasts much longer than the cooling timescale of CREs.
    \item In the primary scenario, the RH emission decays within the cooling timescale ($t_{\rm cool}\approx300~{\rm Myr}$).
    \item The reacceleration boosts the radio power almost two order of magnitude larger. Thus, we can clearly distinguish radio-loud and radio-quiet clusters.
\end{itemize}
%\ers{where the secondary injection is negligible,} 

%\ers{We built the MC merger tree in Section~\ref{sec:MT}. We adopted the merger rate and the median mass accretion rate calibrated with the Millennium simulations, to express the mass evolution through mergers and continuous mass accretion, respectively.} \par

%The initial HMF at $z=0$ is constructed with the fitting formula of \citet{Tinker_2008ApJ...688..709}, and the evolution of each halo is followed to higher redshifts. \par

Based on the merger tree provided in Section~\ref{sec:MT}, we have studied the occurrence conditions of RHs to satisfy the observed RH statistics (Section~\ref{sec:Statis}). The most important update from previous studies is the inclusion of the emission lifetime studied in Section~\ref{sec:lifetime}. We introduce the two conditions for the onset of RHs: {\it mass-ratio condition} and {\it break-frequency condition}. The former condition is expressed with the threshold mass ratio, $\xi_{\rm RH}$, while the latter has two parameters, i.e., the break frequency, $\nu_{\rm b}$, and the fraction of the turbulent energy to the merger kinetic energy, $\eta_{\rm t}$. 

%\ers{A simple power-law is assumed for the relation between peak luminosity and mass, which is characterized with two parameters $\alpha_{\rm M}$ and $A_{\rm RH}$. Those parameters are constrained from the observed RH fraction and the luminosity function.} \par

%\ers{In Section~\ref{sec:X_dynamics}, the method of the mass-ratio condition is applied to study the correlation between RHs and disturbed clusters observed in X-ray. For a given threshold, $\xi_{\rm dyn}$, the total fraction of merging systems in the observed sample constraints the parameter, $t_{\rm relax}$, which is the time required for a disturbed cluster to go back to the relaxed state. We then studied the fraction of RHs in merging systems over total RHs in our merger tree.} \par

%Such small value for $\xi_{\rm RH}$ seems problematic, because $\xi_{\rm dyn}$ should be smaller or comparable to $\xi_{\rm RH}$ considering the tight correlation between RHs and merging systems (Section.~\ref{sec:X_dynamics}). That correlation is compatible with the secondary scenario with $\xi_{\rm dyn}\approx0.1$, and the fraction of RHs residing in relaxed systems would be $10-20\%$. \par 

%\ers{In Section~\ref{sec:origin_of_PM}, we tried to show that the observed steep $P_{1.4}-M_{500}$ could arise from the mass dependence on the reacceleration parameters. We first showed the rapid evolution of the radio luminosity during the reacceleration phase. We then calculated the peak luminosity for various masses, adopting the mass scaling of $t_{\rm acc}\propto M^{-1/3}$ and $t_{\rm R}\propto M^0$. 
%Those mass dependence could be derived under the assumption of binary merger approximation with zero impact parameter (Appendix~\ref{app:Dpp}). 
%Such extension of our model also involves the scaling of other quantities such as the ICM core radius and the turbulent profile.} \par

Our results in Sections~\ref{sec:Statis}-\ref{sec:ASKAP} can be summarized as follows:

\begin{itemize}
    \item The observed fraction and number counts of RHs could be explained in both the two scenarios, but the required threshold value for the merger mass ratio $\xi_{\rm RH}$ differs very much: $\xi_{\rm RH}=0.12$ and $\xi_{\rm RH}=0.01$ are required for the secondary and the primary scenarios, respectively.
    %the secondary scenario requires that RHs should be driven by rare major mergers with , while  for 
    %\item The long lifetime in the secondary scenario requires that RHs should be driven by rare major mergers with $\xi_{\rm RH}>0.25$.
    %\item On the contrary, more frequent onsets by minor mergers ($\xi_{\rm RH}\approx0.01$) are required in the primary scenario.
    
    \item The present Coma RH should be in the middle of the luminosity growth due to the reacceleration. The Coma-like RH would achieve its peak luminosity of $P_{1.4}\approx10^{25}~{\rm W/Hz}$ at an elapsed time $\approx700$ Myr after the onset of the reacceleration.
    % in both the secondary and the primary scenarios.
    
    \item A correlation between the halo mass and the peak radio luminosity is required. This correlation can be reproduced by the mass dependence of the acceleration timescale ($\tau_{\rm acc}\propto M^{-1/3}$) and a constant duration timescale of the reacceleration. Those parameter behaviors can be justified by a simple model as discussed in Appendix~\ref{app:Dpp}.
    
    \item In order to reproduce the tight correlation between the RHs and the dynamical disturbance seen in the X-ray morphology, the threshold mass ratio to induce the merger signature in X-ray observation should be close to $\xi_{\rm RH}$. This condition requires that even minor mergers with a mass ratio $\xi\approx0.01$ should produce observable global disturbances {\bf when the RHs are powered by the reacceleration of primary CREs}.
    
    \item The apparent difficulty in {\bf the reacceleration of primary CREs} can be relaxed if the emission is sustained for a few Gyrs by a gentle reacceleration.
    
    %\item Even for the nearest RH in Coma and the brightest RH in Abell 2744, the secondary model can reproduce the observed properties without conflict with the gamma-ray upper limits.
    
    %\item The RH fraction steeply decreases with decreasing halo mass. However, our model predicts a large number of RHs below the present observable flux limit. The future surveys such as ASKAP are expected to detect $\sim 1000$ RHs below redshift 0.5 for both the secondary and the primary models.
    
    \item The RH fraction steeply decreases with decreasing halo mass. However, our model predicts a large number of RHs below the present observable flux limit. The future surveys such as ASKAP are expected to detect $\sim 1000$ RHs below redshift 0.5, {\bf regardless of whether the radio emission originates from the reacceleration of secondaries or primaries.}
\end{itemize}

%\ers{In Section~\ref{sec:gamma}, we discussed the consistency between our secondary scenario and the gamma-ray limit given by Fermi-LAT, especially for two cluster, Coma and A2744. }
%The former is characterized by its low redshift, $z=0.023$, and it has been reported that the hadronic model cannot consistently explain both the observed radio flux at $\approx300~{\rm MHz}$ and the gamma-ray upper limit by \citet{2014ApJ...796..109A} under the magnetic field constrained from RM \citep[e.g.,][]{Brunetti2017}. 
%\ers{Since the ratio of the low-frequency synchrotron flux to the gamma-ray flux becomes larger by the reacceleration, the tension in the hadronic model of the Coma RH is relaxed by assuming that the RH is in the midst of the reacceleration. The luminosity of the A2744 RH
%\ers{\citep[noted in e.g.,][]{Brunetti2017}}
%is almost 20 times larger than Coma. Its spectrum and brightness profile are well reproduced by the secondary model adopted in
%Section~\ref{sec:origin_of_PM} under the assumption of $B_0=4.7~\mu{\rm G}$ and $t_{\rm R}=t_{\rm R}^{\rm peak}$. We have obtained the constraints on the central field strength, $B_0<0.5~\mu{\rm G}$, which is similar to the previous study} \citep[][]{Jeltema_2011}. \par



%\ers{The prospect for the future survey with ASKAP is discussed in Section~\ref{sec:ASKAP}. The all-sky number count of RHs could rise up to $\approx10^3$. The number count would be dominated by low-mass systems with $M_{500}\approx2\times10^{14}~M_\odot$, which are mostly formed at $z<0.5$. The increased statistics would bring a great impact on both cosmology and high-energy astrophysics, and the improvement in understanding about the origin of RHs would be expected. Limiting the frequency at 1.4 GHz, however, the expected number count and the mass dependence in $f_{\rm RH}$ at 1.4 GHz show similar trends for both scenarios.} \par

%........Since........., a multi-band survey would be important to distinguish the two scenarios. \par

In summary, we have found that both the secondary and primary models for  the origins of the seed CREs are allowed from the current RH statistics. Both the models have both merits and demerits. The secondary scenario requires only major mergers for the RH onset, which is consistent with the fact that RH clusters tend to show observable morphological disturbance. However, for the Coma RH, the secondary model requires a steeper injection spectral index compared to the primary scenario (see Appendix \ref{app:ComaAlpha}). That requirement is even severer for USSRHs, and the CRP energy density possibly exceeds that of the thermal ICM for such RHs in the absence of the reacceleration \citep[e.g.,][]{Brunetti_2008Natur.455..944B}. On the other hand, the primary scenario provides a better fit to the Coma spectrum with a flatter injection index and potentially explains USSRHs without requiring an extremely high CR energy density. However, the short lifetime in this scenario requires frequent onsets with $\xi\approx0.01$ mergers, which is one order of magnitude smaller than the typical value estimated in RH clusters \citep[e.g.,][]{Cassano_2016}. The required efficiency for the turbulence excitation is relatively high in the primary model to explain the acceleration time of $\approx300~{\rm Myr}$ within the formulation of Appendix~\ref{app:Dpp}. {\bf Those difficulties could be relaxed if the RHs are sustained by the reacceleration with a longer timescale.} Either an extended study dedicated for the RH population in lower ($\approx100{\rm MHz}$) and higher frequencies ($\approx10{\rm GHz}$), or a statistical analysis of the merger mass ratio of RHs would further constrain the origin of relativistic electrons in the ICM. \par

%Finally, we note the applicability of our method for future studies that focus on the cosmological evolution of CR contents in the ICM. When the reacceleration is efficient higher energies, as assumed in this study, our demonstration suggests that CRP can work as a reservoir of energy induced by mergers. Since CRPs are well confined in the cluster volume and do not lose their energy through radiative cooling, their energy density would successively increase through sequential mergers. Even if the CRE population is dominated by the primary origin at the early stage of the cluster evolution, the secondary injection could eventually overcome the primary injection at a later epoch. The injection mechanism of CREs, either primary or secondary origin, should depend on the integrated history of mergers and could differ cluster to cluster.  

%This point should be featured in future studies that focus on the cosmological evolution of CR contents in galaxy clusters.



==> trash/DISCUSSION.tex <==
\section{Discussion and Conclusions}
\label{sec:discussion}
Radio observations of the extragalactic background detected the excess over the CMB in $22~{\rm MHz}<\nu<10~{\rm GHz}$.
The origin of this excess emission is still under debate and GCs are the possible candidates  \citep[][]{Fang_2015PhRvD..91h3501F,Fang_Linden:2016dga}.
On the other hand, several studies have shown that GCs can work as reservoir of CRs and make a significant contribution to the high-energy neutrino background observed by IceCube \citep[e.g.,][]{Murase2008,Murase_Waxman2016,Fang_2018NatPh..14..396F,Hussain:2021dqp}.
In this study, we adopt the model constrained from the statistical properties of GRHs and evaluated the contribution from massive ($M_{500}>3\times10^{14}M_\odot$) clusters to those backgrounds.
%examined if the GCs can make the dominant contribution to the radio and neutrino background, considering the statistical properties of GRHs observed in massive clusters.
\par

The observational properties of GRHs, such as coincidence with cluster mergers and steep spectra, are well explained with the re-acceleration of seed CREs by the merger-induced turbulence.
In this study, we assumed that the radio and neutrino emission from GCs are powered by the re-acceleration of CRs.
We adopted so-called secondary scenario, where the seed CREs are provided through the $pp$ collision of CRPs.
We used the merger tree of dark matter halos to calculate the LFs of radio and neutrino emission.
The onset of the re-acceleration is conditioned by the merger mass ratio, and the threshold mass ratio $\xi_{\rm RH}$ is constrained from the observed population of GRHs.
Solving the FP equations, we found that synchrotron and neutrino luminosities rapidly increase with time as modeled with Eqs.~(\ref{eq:h_radio}) and (\ref{eq:h_nu}).
Assuming that the re-acceleration efficiency (modeled with the momentum diffusion coefficient $D_{pp}$) increases with the mass, we found that the peak values of radio and neutrino luminosities increase with cluster mass.  
\par

In our fiducial model, we adopted $B_{\rm radio} = 3.5$ and $B_\nu = 1.67$ for the slope of the radio and neutrino luminosity--mass relations. 
This model fits well the observed statistics of GRHs. 
Due to the relatively steep luminosity--mass relation, massive clusters with $M_{500}>5\times10^{14}M_\odot$ mainly contribute to the backgrounds.
%% multiplet constraint %%
Especially, the effective neutrino luminosity becomes as large as $E_\nu L_\nu\approx10^{42.5}$ erg/s, which corresponds to the mass of $M_{500}=2.0\times10^{15}M_\odot$. 
The number density of such source is as small as $n^{\rm eff}=5.4\times10^{-10}{\rm Mpc}^{-3}$.
\par

We found that the contribution to the ARCADE2 excess is marginal.
This result is at odd with the previous estimate by \citet{Fang_Linden:2016dga}.
We adopted typical luminosity of GRHs, which is more than two orders of magnitude smaller than that assumed in \citet{Fang_Linden:2016dga}.
\par

\kn{Although the total neutrino intensity is only 5\% of the observed one, multiplet events could be expected in this model \citep[][]{Murase_Waxman2016}.
Such model can be tested with the point source search with the sensitivity of 10 yrs search of IceCube-Gen2. ....}

\par

%% statistics of low mass RHs and optimistic model %%%

In the optimistic model, we assumed a shallower luminosity--mass relation, which also can be obtained in the re-acceleration scenario when the efficiency of the re-acceleration is independent of the mass, i.e., $D_{pp}\propto M^0$.
The emission from $M_{500}\approx10^{14}M_\odot$ clusters become most important both for radio and neutrino backgrounds, yet the contribution to the ARCADE2 excess is less than 1\%.
We expect the same level of the neutrino background in this model as previous ``accretion-shock" models, where the same luminosity-- mass relation is adopted \citep[e.g.,][]{Murase2008,Zandanel2015,Murase_Waxman2016,Fang_2018NatPh..14..396F}.

\par

Both our fiducial and optimistic models are consistent with the observed increase of $f_{\rm RH}$ with cluster mass \citep[][]{Cuciti_2015A&A...580A..97C,2021A&A...647A..50C}, but the trend is weaker in the optimistic scenario.
The fiducial scenario predicts that $f_{\rm RH}$ observed with the sensitivity of the Australian SKA Pathfinder (ASKAP) will be $f_{\rm RH}\approx0.05$ in the mass rage of $10^{14}M_\odot<M_{500}<10^{14.5}M_\odot$ \citep[][]{paperII}, while it will be $f_{\rm RH}\approx0.3$ in the optimistic model.
Both models predict $f_{\rm RH}\approx0.6$ around $M_{500}=10^{15}M_\odot$.
Thus, the future survey on GRHs in low mass clusters ($M_{500}<10^{14.5}M_\odot$) will give an important test of our models.

\par

Summarizing above, we conclude that near-by massive clusters are not desirable source for either neutrino or radio backgrounds. 
Our result does not exclude the possibility that GCs with lower masses ($M_{500}<10^{14}M_\odot$) and higher redshifts ($z>0.5$) are the dominant source of neutrino background.
As suggested by previous studies, the GCs in $0.3<z<1$ with masses of $M_{500}\approx10^{14}M_\odot$ can be the dominant source of the neutrino background, when CRs are mainly provided by the outflows from AGNs \citep[e.g.,][]{Fang_Olinto2016,Hussain:2021dqp}.
On the other hand, the recent detection of GRHs in low-mass \citep[][]{Botteon_2021} and high-z \citep[][]{DiGennaro_2021NatAs...5..268D} clusters would suggest that the re-acceleration is efficient in such clusters.
Future studies should follow the log-term evolution of CR distributions, incorporating both the CR injection from AGNs and the re-acceleration.



%Although those calculations have not incorporated the effect of re-acceleration, it can be the case that the re-acceleration is effective only in low redshifts and that the neutrino background is dominated by GCs in relatively high redshifts (say, $z>1$) \footnote{note that the GRHs are detected up to $z\approx0.9$ }.





==> trash/INTRO.tex <==
\section{Introduction\label{sec:intro}} 

%%%%%% ARCADE radio background %%%%%%%
The Absolute Radiometer for Cosmology, Astrophysics, and Diffuse Emission (ARCADE) 2 experiment detected the extragalactic radio background at frequencies 3-90 GHz in excess of the cosmic microwave background radiation (CMB) and the Galactic foreground \citep[][]{ARCADE2_Fixsen_2011ApJ...734....5F}. 
Combined with the observations at lower frequencies \citep[e.g.,][]{Haslam_1982A&AS...47....1H,Reich_1986A&AS...63..205R}, the absolute temperature of the excess emission over the CMB shows a power-law dependence on frequency, $T\propto\nu^{-2.6}$, from 22 MHz to 10 GHz. 
\par

% X-ray background Singal (2010) & anisotropy Holder (2014)
The origin of the ARCADE-2 excess is still under debate. 
The contribution from known radio sources, such as radio galaxies is not sufficient to explain its origin \citep[e.g.,][]{Singal_2010MNRAS.409.1172S,Condon_2012ApJ...758...23C}. 
Considering the synchrotron emission from relativistic electrons, the magnetic field of the source should be larger than $\sim 1\mu{\rm G}$ in order not to overproduce the X-ray and gamma-ray background through the inverse-Compton scattering of the cosmic microwave background (CMB) photons \citep[][]{Singal_2010MNRAS.409.1172S}. 
\par

Considering the observations of the extragalactic sky by the Australia Telescope Compact Array (ATCA) and the Very Large Array (VLA), \citet{Holder_2014ApJ...780..112H} found that the anisotropy of the radio background is lower than that expected from the sources that traces the large scale structure of the universe within $z<5$. 
However, as noted by \citet{Holder_2014ApJ...780..112H} and \citet{Fang_2015PhRvD..91h3501F}, the anisotropy is constrained only for small angular scales ($l>6,000$) since the radio interferometers are insensitive to the emission on larger angular scales. 
Thus, the constraint could be less stringent for large sources like galaxy clusters (GCs).
\par 

% Fang & Linden, galaxy clusters
%\citet{Fang_2015PhRvD..91h3501F} calculated the synchrotron radiation from the electrons produced by through the the dark matters annihilation within the intra-cluster medium. They found that  contribution from the substructure should be large and strong magnetic field ...  

\citet{Fang_Linden:2016dga} showed that the ARCADE-2 excess can be explained by the synchrotron emission from relativistic electrons re-accelerated by the turbulence in merging GCs with reasonable values of the magnetic field ($\sim10\mu{\rm G}$) and the efficiency of the re-acceleration. 
\par



%%%%% IceCube neutrino %%%%%%
Galaxy clusters also draw attention as a possible source class of the background emission of high-energy neutrinos observed by IceCube \citep[][]{IceCube_2013PhRvL.111b1103A}. 
Galaxy clusters can work as cosmic-ray (CR) reservoirs, within which cosmic-ray protons (CRPs) are accumulated over cosmological timescale and emit gamma-ray and neutrinos through the inelastic $pp$ collision with the thermal protons in the intra-cluster medium (ICM). 
\par


Many of previous works compared two possibilities for the origin of CRs in the ICM; ``accretion" shock model and ``internal source" model \citep[e.g.,][]{Murase_Waxman2016}. 
In the accretion shock model, at most $20\%$ of the IceCube flux around 1 PeV can be explained by the emission from massive GCs ($M>10^{15}M_\odot$) \citep[e.g.,][]{Fang_Olinto2016,Hussain:2021dqp}. 
In the internal source models, the CRs are provided through the outflows from active galactic nuclei (AGN) and galaxies inside the cluster. 
In this case, $100\%$ of the IceCube flux can be achievable \citep[e.g.,][]{Fang_Olinto2016,Fang_2018NatPh..14..396F,Hussain:2021dqp}. 
%The latter scenario is compatible with the source density constraints from the analysis of multiplet events in the IceCube data \citep[][]{Murase_Waxman2016}. 
%the CR production rate is assumed to scale the cluster mass as $M^{5/3}$, and 
%, and its production rate is proportional to $M$
%the contribution is dominated by GCs in mass range of $10^{14}M_\odot<M<10^{15}M_\odot$ and
\par


%Based on this scenario, \citet{Fang_2018NatPh..14..396F} showed that the observed flux of the neutrino background, the gamma-ray background, and the ultra-high energy cosmic-ray, simultaneously. The contribution to the neutrino background is dominated by the clusters in mass range of $10^{14}M_\odot<M<10^{15}M_\odot$. 


%%%%% GRH & reacceleration %%%%%%%%
Meanwhile, the direct evidence for the existence of the relativistic particles in the ICM has been achieved only with the radio observations.
A fraction of clusters host extended radio structures, such as giant radio halos (GRHs), mini halos, and radio relics \citep[][]{review_vanWeeren}. 
\par

The Mpc-scale extension of GRHs can be explained by in-situ injection and/or acceleration of cosmic-ray electrons (CREs) in the ICM \citep[][]{Brunetti_Jones_review}. 
The tight correlation between cluster merger and GRH supports the re-acceleration scenario, where the non-thermal electrons are re-energized by the stochastic interaction with the merger-induced turbulence permeating the cluster volume. 
The secondary (hadronic) origin of the relativistic electrons is less favored due to the non-detection of gamma-rays from GCs \citep[e.g.,][]{Ackermann2016_cluster} and the existence of the GRHs with very steep spectral indexes $\alpha_{\rm syn}<-1.5$ \citep[e.g.,][]{Brunetti_2008Natur.455..944B}.
%GRHs tend to show steep spectral indexes $\alpha_{\rm syn}\approx-1.5$, which can also be reproduced with the turbulent re-acceleration.  
\par
%Although the secondary (hadronic) origin of the relativistic electrons is less favored by the non-detection of gamma-rays from GCs,
However, it is still possible that the ``seed" electrons for the re-acceleration is provided by the hadronic ($pp$) process. 
Such model is compatible with the observed spectrum and profile of the GRH in the Coma cluster without overproducing the gamma-ray \citep[e.g.,][]{Brunetti2017,Pinzke2017,paperI}.
In \citet{paperII}, we have shown that this model is also consistent with the statistical properties of GRHs, although the condition of the onset of the re-acceleration is significantly different from the ``primary model", where the seed electrons are provided independently of the CRP population.
\par

\citet{Zandanel2015} for the first time constrained the contribution to the IceCube flux from galaxy clusters using the statistics of GRHs in National Radio Astronomy Observatory Very Large Array sky survey (NVSS) and found an upper limit of $\approx10\%$.
We obtained a similar result from an order of magnitude estimate \citet{paperI}, considering that the Coma-like clusters with masses of $M_{500}\approx8\times10^{14}M_\odot$ contribute most, where $M_\Delta$ is the mass within which the average of the total mass density becomes $\Delta$ times the critical density of the Universe.
Due to the limited sensitivity of the radio observations, the current statistics of GRHs is mostly for massive ($M_{500}>3\times10^{14}M_\odot$) systems.
\par


%The missing piece in this turbulent re-acceleration scenario is the origin of seed electrons for reacceleration. In our previous study, .

%% this work
In this paper, we discuss the contribution from massive GCs to the radio and neutrino backgrounds, considering the time evolution of luminosities through the merger history of GCs. 
We adopt the method of \citet{paperII} and utilize the merger tree of dark matter halos built with a Monte Carlo method (Section~\ref{sec:LF}).
With semi-analytic models of luminosity evolution and luminosity--mass relation in the re-acceleration scenario, we construct the luminosity functions (LFs).
Throughout this study, we assume that the seed electrons for the re-acceleration are provided as secondaries of the $pp$ collision to achieve an optimistic result for the high-energy neutrino emission.
Our model parameters are constrained from the statistical properties of GRHs.
In Section~\ref{sec:contribution_backgound}, we show that the contribution to the ARCADE2 excess is sub-dominant. 
The contribution to the IceCube flux around 1 PeV is as large as $\approx5\%$, while it increase to $\approx20\%$ with an optimistic assumption on the neutrino luminosity--mass relation, which is hardly constrained by observations.
In Section~\ref{sec:discussion}, we compare our results with previous estimates and discuss the possible constraints with future radio and neutrino observations.
\par

We adopt the flat $\Lambda$CDM cosmology with the parameters from \citet{Planck18}, where $H_0 = 67~{\rm km/s/Mpc}$ ($h = 0.67$ or $h_{70} = 0.96$). 
\par

%During the structure formation of galaxy clusters, a part of the gravitational potential energy would be dissipated into the acceleration of relativistic particles by the merger. In the so-called turbulent reacceleration model, RHs originate from the reacceleration of seed cosmic-ray electrons (CREs) by the merger-induced turbulence \citep[e.g.,][]{Brunetti_2001MNRAS.320..365B,Petrosian_2001ApJ...557..560P,Fujita_2003ApJ...584..190F}. As the turbulence could permeates the most of the cluster volume, this model can explain the large extension of the radio emission. This model is supported by the observational signature of the turbulence acceleration such as the steep spectral index ($F_\nu\propto\nu^{-\alpha_{\rm syn}}$ with $\alpha_{\rm syn}\approx1.5$) or the break feature in the radio spectrum \citep[e.g.,][]{Brunetti_2008Natur.455..944B,Macario_2010A&A...517A..43M,Wilber_2018MNRAS.473.3536W,DiGennaro_2021NatAs...5..268D}. However, the origin of the seed electrons for the reacceleration has not been revealed yet \citep[e.g.,][]{Brunetti2014}.  \par 

















%% radio halo %%


%\footnote{\url{http://www.lofar.org}}
%% observational facts %%
%A variety of statistical properties of RHs have been reported. For example, the occurrence of RHs correlates with the dynamical disturbance of clusters observed in X-ray \citep[e.g.,][]{Schuecker_2001A&A...378..408S,Cassano_2010_LOFAR,Cassano_2013ApJ...777..141C,2021A&A...647A..50C}, and the radio luminosity is known to correlate with the X-ray luminosity or the mass measured with the Sunyaev-Zel'dovich (SZ) effect \citep[e.g.,][]{Cassano_2013ApJ...777..141C}. In addition, those correlations show bimodalities, as the clusters without RHs fall well below the relations \citep[][]{Brunetti_2007ApJ...670L...5B}. The occurrence of RHs seems to increase with the mass of the cluster \citep[][]{Cuciti_2015A&A...580A..97C,2021A&A...647A..50C}. Those facts indicate a firm connection between the formation process of galaxy clusters and the non-thermal components in the intra-cluster medium (ICM).  \par


%% re-acceleration model %%


%There are two possible origins of the seed CREs. One is the {\it primary} scenario, where CREs are directly injected by accelerators like large-scale accretion shocks, or escaped from radio jets launched from the central active galactic nuclei (AGNs) \citep[e.g.,][]{Kang_2012ApJ...756...97K,Volk_1999APh....11...73V,Gitti_2002A&A...386..456G,Heinz_2006MNRAS.373L..65H}. The other is the {\it secondary} scenario, where the primary CRE injection is dominated by the secondary injection from the pp collisions between cosmic-ray protons (CRPs) and thermal protons in the ICM \citep[e.g.,][]{Brunetti2005,Brunetti2011,Pinzke2017}. Recently, by modeling the well-studied RH in the Coma cluster, we have found that the non-thermal properties, such as the CR energy density and the location of the primary CR accelerators, could be significantly different between those two scenarios, which could be a clue to reveal the seed origin \citep[][]{paperI}. In this study, we further discuss possible differences appearing in the statistics of RHs. \par





==> trash/METHOD.tex <==
%\section{Order Estimate}
%\label{sec:Order_estimate}
%We first discuss the contribution to the ARCADE-2 excess and the IceCube neutrino from massive clusters, using a simple order of magnitude estimate.
%The intensity of the background emission can be roughly estimated from the source number density and the typical luminosity. 

%\begin{eqnarray}
%I_{\nu} \sim \frac{c}{4\pi}\xi_zt_{\rm H}n_{s}L_{\nu},
%\end{eqnarray}


%\subsection{ARCADE-2 Excess}
%We see that the contribution from massive GCs is only marginal, regardless of the origin of the seed electron. Note that the radio luminosity assumed in \citet{Fang_Linden:2016dga} , 3 orders of magnitude larger than observed GRH luminosity, which resulted in a very optimistic estimate. \par

%For the neutrino background, we have estimated the . \par

%\subsection{Neutrino Background}
\section{Merger Tree and Luminosity Function}\label{sec:LF}
We construct the LFs of radio and neutrino emission from galaxy clusters, considering the re-acceleration of CRs by merger induced turbulence. 
We follow the procedure explained in \citet{paperII}, and use the merger tree of dark matter halos built with a Monte Carlo simulation.
As a initial condition, we set up 4,000 halos at $z=0$ following the mass function of \citet[][]{Tinker_2008ApJ...688..709}.
We use the merger rate and (median) mass accretion rate given by \citet[][]{Fakhouri_2010MNRAS.406.2267F} to follow the mass evolution of each halos.
Our method can reproduce the mass function above $M_{500}>10^{12}M_\odot$ at redshift up to $z=5$.
\par

In Sect.~\ref{subsec:L_evolution}, we explain our model to calculate the radio and neutrino luminosities of each halo.
In Sect.~\ref{subsec:model_parameters} we discuss the constraints on our model parameters from the observation of GRHs.
In Sect.~\ref{subsec:LF}, we show the results.

\subsection{Luminosity Evolution in Re-acceleration Model}
\label{subsec:L_evolution}
The emission luminosity of each halo is calculated depending on its merger history.
We assume that the re-acceleration of CRs starts with mergers that satisfies the condition, $\xi>\xi_{\rm RH}$, where $0<\xi<1$ is the mass ratio of the merger and $\xi_{\rm RH}$ is the threshold value.
The luminosity is determined as a function of the mass of the halo $M_{500}$ and the time since the re-acceleration starts $t_{\rm R}$, $L=L(M_{500},t_{\rm R})$. 
\begin{eqnarray}
\left(\frac{L(M_{500},t_{\rm R})}{L_0}\right) = 10^{A}\left(\frac{M_{500}}{M_0}\right)^{B}h(t_{\rm R}),
\label{eq:Luminosity_model}
\end{eqnarray}
where $L_0$ is the typical luminosity for the mass $M_0$, $A$ and $B$ are model parameters for the peak luminosity achieved by re-acceleration, and the function $h(t_{\rm R})$ denotes the time evolution.
The peak of the luminosity is achieved at $t_{\rm R} = t_{\rm R}^{\rm peak}$, i.e., $h(t_{\rm R}^{\rm peak})=1$.
In the following, we distinguishes the quantities for radio and neutrino emission using the subscript, e.g., $L_{\rm radio}$ for radio luminosity and $L_\nu$ for neutrino luminosity.
For a prompt comparison with observations, $L_{\rm radio}$ is expressed in the unit of [W/Hz], while $L_\nu$ is in [GeV/s/GeV] (the number luminosity per unit energy multiplied by the energy).
We adopt $(L_0,M_0) = (10^{24.5}~{\rm W/Hz},10^{14.9}~M_\odot)$ for radio, and $(L_0,M_0) = (10^{40}~{\rm GeV/s/GeV},10^{15}~M_\odot)$ for neutrino.
\par


As discussed in \citet{paperII}, the temporal evolution of the luminosity and the best fit values for the model parameters depend on the origin of the seed electrons; secondary or primary. 
To achieve the most optimistic estimate on the neutrino background, we assume that all of the seed electrons are produced through the $pp$ collision, i.e., same as the ``secondary scenario". \par


\begin{figure}
    \centering
    \plotone{figures/L_time_radio_nu.pdf}
    \caption{Time evolution of synchrotron luminosity at 1.4 GHz (red thick line) and neutrino luminosity at 100 TeV (blue thin line). Those trends are modeled with $h(t_{\rm R})$ (Eqs.~(\ref{eq:h_radio}),(\ref{eq:h_nu})). The re-acceleration starts at $t_{\rm R}=0$ and ends at $t_{\rm R} = t_{\rm R}^{\rm peak}$ (dashed line).}
    \label{fig:L_time}
\end{figure}

We follow the time evolution of the CR spectra during and after the re-acceleration by solving the Fokker--Planck (FP) equations \citep[e.g.,][]{Brunetti2005,Fujita_2003ApJ...584..190F,paperI}:
\begin{eqnarray}
\frac{\partial N_{s}}{\partial t} &=& \frac{\partial}{\partial p}\left[N_{s}\left(b_s -\frac{1}{p^2}\frac{\partial}{\partial p}(p^2D_{pp})\right)\right]+\frac{\partial^2}{\partial p^2}[D_{pp}N_s] \nonumber \\
&&+Q_s-T_s,
\label{eq:FokkerPlanck}
\end{eqnarray}
where $N_{s}$ is the phase space number density of particle species $s$, $b_{s}$ is the momentum loss rate ($b\equiv\frac{dp}{dt}$), $Q_{s}$ is the injection term, and $T_{s}$ is the sink term.
We consider the radial dependence, i.e., $N_s = N_s (r,p,t)$, although we neglect the effect of the radial diffusion for simplicity.
\par

For the terms appear in Eq.~(\ref{eq:FokkerPlanck}), we adopt the assumption made in Section 7 of \citet[][]{paperI}.
The momentum loss rate of CRPs $b_p$ includes the effect of the Coulomb collision with thermal electrons and thermal protons \citep[][]{Petrosian2015}.
Both the Coulomb cooling and the radiative cooling due to synchrotron and inverse-Compton (IC) radiation are included in the loss rate of CREs $b_{e}$.
The re-acceleration is modeled with the momentum diffusion coefficient $D_{pp}$.
We assume the hard-sphere type re-acceleration, i.e., $D_{pp}\propto p^2$, with a mass dependence of $D_{pp}\propto M^{1/3}_{500}$.
We also consider the radial dependence of $D_{pp}$ and adopt the profile as \citet[][]{paperII}, which fits well the observed radio profile of the Coma cluster at 350 MHz.
For the mass of the Coma cluster ($M_{500} = 8.5\times 10^{14}M_\odot$), the acceleration timescale $t_{\rm acc}=p^2/(4D_{pp})$ becomes $t_{\rm acc} = 330~{\rm Myr}$ at $r = r_{\rm c}$, where $r_{\rm c}$ is the core radius of the beta-model profile of the ICM \citep[e.g.,][]{Briel_1992A&A...259L..31B}.
The CR injection term $Q_{p}$ shares the same profile as the ICM energy density.
The injection spectrum is $Q_{p}\propto p^{-\alpha_{\rm inj}}$ with $\alpha_{\rm inj} = 2.45$, which can reproduce the typical spectral index of GRHs. 
We neglect the injection of the primary CREs ($Q_{e} \equiv 0$).
The loss of CRPs due to the inelastic $pp$ collision is expressed with the sink term as $T_p = N_p/\tau_{pp}$, where $\tau_{pp}$ is the timescale for $pp$ loss \citep[][]{paperI}.
For CREs, we adopt $T_e \equiv 0$.
%We adopt the cross section for the pp collision given by \citet{Kamae2006} and the secondary neutrino spectrum given by \citet{Kelner2006}.
\par

To discuss the luminosity--mass relation, we consider the mass dependence of physical quantities.
The observed temperature--mass relation \citep[][]{Vikhlinin_2006ApJ...640..691} is s adopted for the ICM temperature.
The core radius of the ICM distribution is scaled with the virial radius, $r_{\rm c} = 0.2R_{500}$.
The re-acceleration efficiency increases as $D_{pp}\propto M^{1/3}$, while the duration of the re-acceleration is assumed to be constant $t_{\rm R}^{\rm peak}\propto M^{0}$.
We adopt the magnetic field profile of the Coma cluster measured with the Faraday Rotation Measure \citep[][]{Bonafede2010} and do not consider any mass dependence in the field strength $B_0$ and the profile $\eta$.
\par

Figure~\ref{fig:L_time} shows the time evolution of the synchrotron luminosity at 1.4 GHz (red line) and the all-flavor neutrino luminosity at 100 TeV (blue line) during and after the hard-sphere type re-acceleration. 
Both luminosities increase with time during the re-acceleration, but the steepness of the increase is different.
The synchrotron emission during the re-acceleration is supported by both the re-acceleration of pre-deposited secondary CREs and the fresh injection from the re-accelerated cosmic-ray protons (CRPs) \citep[see][for detail]{paperII}.
The GHz emission is mainly produced by CREs with $\sim{\rm GeV}$ energies, which is produced through the $pp$ collision of $\sim10~{\rm GeV}$ CRPs.
The Coulomb cooling between CRPs and the ICM suppress the re-acceleration of GeV CRPs, while higher energy CRPs are efficiently accelerated without cooling.
Thus, the luminosity of 100~TeV neutrino evolves more rapidly than the GHz radio luminosity (see also Figure~2 of \citet{paperI}).
Note that the power of GeV gamma-ray evolves with a similar rate as the radio luminosity.
\par
 
The radio flux around 1 GHz decays after the re-acceleration, which is due to the radiative cooling of re-accelerated CREs.
The fresh injection from CRPs still supports the radio power after the re-acceleration.
On the other hand, the neutrino luminosity do not decay after the re-acceleration, since the parental CRPs ($E>1$ PeV) do not suffer from significant cooling processes. 
\par

We model the luminosity evolution explained above, using the function $h(t_{\rm R})$. Its functional form for synchrotron and neutrino emission becomes
\begin{eqnarray}
h_{\rm radio}(t_{\rm R})&=&
\left\{
\begin{array}{cc}
    10^{2.0\left(\frac{t_{\rm R}-t_{\rm R}^{\rm peak}}{t_{\rm R}^{\rm peak}}\right)} & (t_{\rm R}-t_{\rm R}^{\rm peak}<0), \\
    \exp\left[-\frac{t_{\rm R}-t_{\rm R}^{\rm peak}}{t_{\rm cool}(z)}\right] & (0<t_{\rm R}-t_{\rm R}^{\rm peak}<t_1), \\
    \exp\left[-\frac{t_1-t_{\rm R}^{\rm peak}}{t_{\rm cool}(z)}\right] & (t_1 < t_{\rm R}-t_{\rm R}^{\rm peak}),
\end{array}
\right.\\
\label{eq:h_radio}
h_{\nu}(t_{\rm R})&=&
\left\{
\begin{array}{cc}
    10^{3.5\left(\frac{t_{\rm R}-t_{\rm R}^{\rm peak}}{t_{\rm R}^{\rm peak}}\right)} & (t_{\rm R}-t_{\rm R}^{\rm peak}<0), \\
    1 & (0<t_{\rm R}-t_{\rm R}^{\rm peak}),  
\end{array}
\right.
\label{eq:h_nu}
\end{eqnarray}
where $t_{\rm cool}(z)$ is the cooling time of CRE at the energy corresponding to 1.4 GHz, and $t_1 = 1.4t_{\rm cool}(z)$ \citep[see][for the detail]{paperII}.
Following \citet[][]{paperII}, We adopt $t_{\rm R}^{\rm peak}=600~{\rm Myr}$.
\par

%For simplicity, we assume the same spectral shape for all clusters in merger tree. 
%We adopt the spectral shape of the Coma cluster the as a template \citep[][]{paperI}.
%The spectral index of the primary CR is assumed to be $\alpha_{\rm inj} = 2.45$.
%\par

\subsection{Model Parameters}
\label{subsec:model_parameters}
The radio power of GRHs correlates with the mass of the host clusters \citep[e.g.,][]{Cassano_2013ApJ...777..141C,2021A&A...647A..50C}. 
Following our previous study, we include the mass dependence of the peak luminosity achieved by re-acceleration (Eq.~(\ref{eq:Luminosity_model})).
The parameters $(A_{\rm radio}, B_{\rm radio})$ and $\xi_{\rm RH}$ can be constrained from the occurrence of the GRHs $f_{\rm RH}$ and its mass trend \citep[][]{paperII}.
\par

We first adopt the same set of parameters as \citet{paperII}, i.e., $(A_{\rm radio}, B_{\rm radio})=(0.6, 3.5)$.
In the following, this model is termed as ``fiducial model" (Table~\ref{tab:params}).
We also consider an ``optimistic model" with a shallower luminosity--mass relations than the fiducial model (Section~\ref{subsec:LF}).
\par

\begin{table}[h]
    \centering
    \caption{Parameters for fiducial model (fid.) and optimistic model (opt.).}
    \begin{tabular}{cccc}
    \hline
      model   & $\xi_{\rm RH} $ & $(A_{\rm radio}, B_{\rm radio})$ & $(A_\nu, B_\nu)$\\
      \hline
       fid.  &  0.12 & (0.6, 3.5) & (0.93, 4.67) \\
       opt.  & 0.30 & (0.6, 2.0)  &  (0.73, 1.67)  \\
    \hline
    \end{tabular}
    %\tablecomments{The parameters $(A_{\rm radio},B_{\rm radio})$ and $(A_\nu,B_\nu)$ are for Eq.~(\ref{eq:})}
    \label{tab:params}
\end{table}

The steep trend between $L_{\rm radio}$ and $M_{500}$ could be explained in the models where the re-acceleration is more efficient in mergers of more massive clusters \citet[][]{Cassano_2012,paperII}.
Since the luminosity depends on $t_{\rm R}$ (see Figure~\ref{fig:L_time}), we focus on its maximum value.
In \citet{paperII}, we showed that the steep relation between the peak luminosity and $M_{500}$ can be reproduced when the re-acceleration efficiency scales with mass as $D_{pp}\propto M^{1/3}$ and $t_{\rm R}^{\rm peak}$ is independent of the mass. 
The acceleration timescale scales as $t_{\rm acc}=p^2/(4D_{pp})\propto M^{-1/3}$.
We neglected possible $\xi$ dependence of $D_{pp}$, assuming that most of the observed GRHs are driven by the near-threshold mergers, $\xi\simeq\xi_{\rm RH}$.
We solved the FP equation for clusters with different masses, and fitted the relation between peak luminosity and mass with Eq.~(\ref{eq:Luminosity_model}). 
We reported the best fit values for the parameters; $(A^{\rm fit}_{\rm radio}, B^{\rm fit}_{\rm radio})=(0.49, 2.83)$.
\par

Using the same procedure, we can obtain the theoretical relation between the neutrino luminosity $L_{\nu}$ and the mass $M_{500}$.
We find the best fit values of $(A^{\rm fit}_\nu,B_\nu^{\rm fit})=(0.93, 4.67)$.
The mass dependence $B^{\rm fit}_{\nu}$ is steeper than $B^{\rm fit}_{\rm radio}$ due to the following two reasons; $L_\nu$ more steeply increases with $t_{\rm R}/t_{\rm acc}$ than $L_{\rm radio}$ (Figure~\ref{fig:L_time}) and $t^{\rm peak}_{\rm R}/t_{\rm acc}$ increase with $M_{500}$.
The evolution of $L_\nu$ in the merger tree is calculated with $(A_\nu, B_\nu) = (0.93,4.67)$ in our fiducial model.
\par


\subsection{Luminosity Functions}
\label{subsec:LF}
For a given set of $(A_{\rm radio},B_{\rm radio})$ and $h_{\rm radio}(t_{\rm R})$, we can constrain $\xi_{\rm RH}$ from the observed occurrence of GRHs.
For the clusters observed with NVSS, and the extended GMRT Radio Halo Survey, the occurrence becomes $\approx30\%$, i.e., $f_{\rm RH}\approx0.3$, for $M_{500}>3\times10^{14}M_\odot$ \citep[e.g.,][]{Kale_2013A&A...557A..99K,2021A&A...647A..50C}.
Adopting the sensitivity of those observations, we calculate $f_{\rm RH}$ at a given range of redshift.
Since the merger rate scales with $\xi^{-2}$ \citep[e.g.,][]{Fakhouri_2010MNRAS.406.2267F}, smaller $\xi_{\rm RH}$ leads to larger $f_{\rm RH}$, and vice versa.
In \citet{paperII}, we found that $\xi_{\rm RH}\approx0.1$ well reproduces the observed $f_{\rm RH}$ in our fiducial model.
\par


To discuss the upper limit for the contribution to the ARCADE-2 excess, we test the ``optimistic model" with shallower $B_{\rm radio}$.
The radio luminosity--mass relation is normalized at the mass of $M_{500}=10^{14.0}M_\odot$, so a shallower luminosity-mass relation predicts larger contribution from smaller mass clusters, such as $M_{500}\simeq10^{14}M_\odot$, which are not yet well constrained observationally.
We adopt $(A_{\rm radio},B_{\rm radio})=(0.6,2.0)$ in the optimistic model. 
We find that those parameters are only marginally consistent with the observed increase of $f_{\rm RH}$ with respect to $M_{500}$ in the range of $5\times10^{14}M_\odot<M_{500}<10^{15}M_\odot$ \citep[][]{2021A&A...647A..50C}.
\par

We find that a luminosity--mass relation similar to $L_{\rm radio}\propto M^{2.0}$ can be reproduced in the model with constant acceleration efficiency with respect to the mass, i.e., $D_{pp}\propto M^0$.
Assuming $t_{\rm R}^{\rm peak}=600~{\rm Myr}$,  the peak luminosity can be fitted with Eq.~(\ref{eq:Luminosity_model}) with $(A^{\rm fit}_{\rm radio},B^{\rm fit}_{\rm radio}) = (0.69,1.78)$.
\par

In our calculation, the CR injection rate is scaled with the cluster mass as $Q_p\propto M^{2/3}$ (Section~\ref{subsec:L_evolution}). 
Besides, we implicitly consider the calorimetric limit for $pp$ collision, neglecting the effect of spatial diffusion.
Thus, the neutrino luminosity should scale as $L_\nu \propto M^{5/3}$ when the other parameters are independent of the mass
\citep[e.g.,][]{Keshet:2002sw,Murase2008,Zandanel2015}.
We confirm that the above scaling is well reproduced in our calculation, so we adopt $B_\nu=5/3$ in the optimistic model (Table~\ref{tab:params}).
The parameter $A_\nu=2.93$ is obtained for $t_{\rm acc}^{\rm peak}=600$~Myr.
For the synchrotron emission, $B^{\rm fit}_{\rm radio}$ slightly deviates from 5/3, which might be due to the re-acceleration of seed electrons.
\par

With a shallower $B_{\rm radio}$, the optimistic model tend to produce many observable GRHs in the low-mass bin ($5\times10^{14}M_\odot<M_{500}<8\times10^{14}M_\odot$).
Thus, a slightly larger $\xi_{\rm RH}$ is required to fit the observed $f_{\rm RH}$ in this mass bin.
We summarize the values of model parameters in Table~\ref{tab:params}.
\par


\begin{figure*}
    \centering
    \plottwo{figures/radio_LF_eff.pdf}{figures/nu_LF_eff.pdf}
    \caption{Luminosity functions for radio (1.4 GHz) and neutrino (100 TeV) emission in the fiducial model. The LFs are multiplied by the luminosity. We show the redshift evolution from $z =1$ to $z=0$ (every 0.2, from red to blue). The dashed lines show the luminosities corresponding to the mass $M_{500} = 10^{13}M_\odot,10^{14}M_\odot$, and $10^{15}M_\odot$ calculated with the $L-M$ relation at $z=0$.}
    \label{fig:LF}
\end{figure*}


In Figure~\ref{fig:LF}, we show the LFs for the synchrotron (1.4~GHz) and neutrino emission (100~TeV) in the fiducial model. 
The LFs are multiplied by the luminosity ($L_{1.4}$ or $L_\nu$) so that one can see the relative contribution from each luminosity bin to the isotropic background.
Different colors show the LFs at different redshifts between $0<z<1$ (every 0.2).
The dashed lines show the typical luminosity corresponding to the masses $M_{500}=10^{14}M_\odot$ and $10^{14}M_\odot$ at $z=0$.
We can define the effective luminosity, $L^{\rm eff}$, as the luminosity that maximize $L(dN/dV_{\rm c}d\log L)$ \citep[e.g.,][]{Murase_Waxman2016}.
We see that the effective luminosity for the radio background is $L^{\rm eff}_{1.4}=10^{24.5}~{\rm W/Hz}$ at $z=0$, which is the typical luminosity of GRHs in the clusters with masses similar to Coma, $M_{500}\approx8.5\times10^{14}M_\odot$. 
Due to the steeper mass--luminosity relation for neutrino, the effective luminosity at 100 TeV becomes $E_\nu L_\nu^{\rm eff}=10^{42.5}~{\rm erg/s}$, which corresponds to $M_{500}=2.0\times10^{15}M_\odot$.
The effective source number density is $n^{\rm eff}_{\nu} = 5.4\times10^{-10}~{\rm Mpc}^{-3}$.
\par
%This mass is larger than the cut-off mass of the halo mass function, which means that the contribution is dominated by very rare systems.

%% optimistic model %%
In the optimistic model, we find $L_{\rm radio}^{\rm eff}=~10^{23.8}$ W/Hz and $E_\nu L_{\nu}^{\rm eff}=~10^{39.5}$ erg/s.
Those luminosities correspond to the mass of $M_{500} = 1.4\times10^{14}M_\odot$.
The effective source number density for the neutrino background becomes $n^{\rm eff}_{\nu}=1.0\times10^{-6}~{\rm Mpc}^{-3}$.
%As expected,.


\section{Contribution to Background Emission}
\label{sec:contribution_backgound}
In this section, we discuss the contribution from massive GCs to the isotropic background of radio and neutrino emission, using the LFs shown in the previous section.
Our method in the previous section only gives the flux at a given frequency (or energy). 
For the spectrum, we assume that all the clusters share the same spectral shape as Coma, which is modeled in \citet[][]{paperI}.
We do not include any redshift or mass dependence in the spectral shape.
Note that the spectral index of the Coma GRH below 1.4 GHz, $\alpha_{\rm syn}=-1.22$, is typical among the observed population \citep[e.g.,][]{Brunetti_Jones_review,review_vanWeeren}.
The luminosities at 1.4 GHz and 100 TeV are used to normalize the spectra of synchrotron and neutrino emission, respectively.
\par

The intensity of the isotropic background ($dN/d\nu dtdAd\Omega$) can be calculated as
\begin{eqnarray}
\Phi_\nu & = &\frac{1}{4\pi}\int dz \frac{dV_{\rm c}}{dz}\int dL_{\rm \nu_{\rm i}} \frac{dN}{dL_{\nu_{\rm i}}dV_{\rm c}}L_{\nu_{\rm i}}\frac{(1+z)^2}{4\pi D_{\rm L}^2(z)}e^{-\tau(\nu,z)}, \nonumber \\
& = & \frac{1}{4\pi}\int dz \frac{c}{H(z)}\int dL_{\nu_{\rm i}}\frac{dN}{dL_{\nu_{\rm i}}dV_{\rm c}}L_{\nu_{\rm i}}e^{-\tau(\nu,z)},
\end{eqnarray}
where $V_{\rm c}(z)$ is the comoving volume, $\nu_{\rm i} = (1+z)\nu$ is the frequency at the source, $\frac{dN}{dL_{\nu_{\rm i}}dV_{\rm c}}$ is the luminosity function, $D_{\rm L}(z)$ is the luminosity distance, and $\tau(\nu,z)$ is the optical depth.
We adopt $\tau(\nu,z)=0$ for the radio and neutrino backgrounds, while we consider the attenuation of gamma-rays by the intreation with the extragalactic background light (EBL) (Section~\ref{subsec:IceCube}). 
For the neutrino background, we calculate the intensity per unit energy ($dN/dEdtdAd\Omega$) rather than that per unit the frequency.
\par

\subsection{ARCADE-2 Excess}
\label{subsec:ARCADE}
\begin{figure}
    \centering
    \plotone{figures/EGRB_Tb_res.pdf}
    \caption{The isotropic radio background expected from galaxy clusters. The solid and dashed lines show the results of the fiducial and the optimistic models, respectively. The data points show the measured radio background after subtracting off the CMB temperature \citep[][]{ARCADE2_Fixsen_2011ApJ...734....5F}.}
    \label{fig:ARCADE2}
\end{figure}

In Figure~\ref{fig:ARCADE2}, we compare the spectrum of the radio background from galaxy clusters with the ARCADE-2 excess.
We see that the contribution is not important for all frequencies between $0.01~{\rm GHz}<\nu<10~{\rm GHz}$.
This result is in contrast to the previous estimate by \citet[][]{Fang_Linden:2016dga}. 
Similar to our result, massive clusters dominate the radio background in their calculation.
However, they assumed larger radio luminosity for each cluster than our models.
Assuming the magnetic field strength $B_0 = 10\mu$G and the fraction of the turbulent velocity to the infall velocity $\eta_v = 0.8$, their model predicts the radio luminosity of $L_{\rm radio}=10^{43}$ erg/s, which corresponds to $L_{1.4}= 10^{26.5}$ W/Hz when the minimum frequency of the synchrotron emission is $\sim1$ MHz. 
This luminosity is almost two orders of magnitude larger than the typical luminosity of the GRHs \citep[e.g.,][]{Cassano_2013ApJ...777..141C}.
Considering the statistical properties of  GRHs, we conclude that massive galaxy clusters cannot be the dominant source of the ARCADE-2 excess.
\par


\subsection{IceCube neutrino}
\label{subsec:IceCube}
\begin{figure}
    \centering
    \plotone{figures/neutrino_bkgd.pdf}
    \caption{The spectrum all-flavor high-energy neutrino background. The data points show the all-sky neutrino intensity of IceCube cascade events \citep[][]{Aartsen_2020PhRvL.125l1104A}.}
    \label{fig:IceCube}
\end{figure}

In Figure~\ref{fig:IceCube}, we show the contribution to the isotropic neutrino background.
The expected flux becomes $\approx5\%$ of the observed intensity around 100 TeV in the fiducial model, while it reaches $\approx18\%$ in the optimistic model.
Those values are comparable or larger than our previous estimate \citep[][]{paperI}, where we only considered the contribution from Coma-like clusters ($M_{500}=8.5\times10^{14}M_\odot$).
%%%Since the effective luminosity $L_\nu^{\rm eff}$ is similar to the luminosity of Coma-like clusters in the fiducial model, 
\par

The expectation in our optimistic model is similar to the one in so-called ``accretion-shock" model \citep[][]{Murase2008,Fang_Olinto2016,Hussain:2021dqp}, where the same luminosity--mass relation ($L_\nu\propto M^{5/3}$) is assumed.
We showed that the radio luminosity should follow a similar to the mass ($L_\nu\propto M^{2}$) when the emission is driven by the re-acceleration and that such model is only marginally consistent with the current statistics of GRHs (Section~\ref{subsec:L-M_rel}).
We can conservatively conclude that the neutrino emission from massive clusters can make up $\approx5\%$ of the isotropic neutrino background.
In Section~\ref{sec:discussion}, we discuss the possible test of our models, using the predicted value of $f_{\rm RH}$ in the future GRH survey.
\par


We also calculated the isotropic gamma-ray background, adopting the optical depth of EBL attenuation given by \citet{Dominguez_2011MNRAS.410.2556D}.  
We have confirmed that both fiducial and optimistic models do not overproduce the non-blazar component of the extragalactic gamma-ray background observed by Fermi-LAT \citep[][]{Ackermann_PhysRevLett.116.151105}.


%In the fiducial model, the contribution from more massive clusters is enhanced by the steep luminosity-mass relation ($B_\nu = 4.67$).

%In \citet[][]{paperII}, we assumed that the Coma RH is in the middle of the re-acceleration phase and has not achieved the peak luminosity for its mass.

%As a result, the background emission is dominated by very massive clusters ($M>$) with very large luminosity($L>$), whose number density is very small ($n<$). 


%We find that the contribution from $z>0.2$ is two orders of magnitude smaller than that from $z\leq0.2$.
